Context-Aware Search and Retrieval Under Token Erasure

This paper introduces and analyzes a search and retrieval model for RAG-like systems under {token} erasures. We provide an information-theoretic analysis of remote document retrieval when query representations are only partially preserved. The query is represented using term-frequency-based features, and semantically adaptive redundancy is assigned according to feature importance. Retrieval is performed using TF-IDF-weighted similarity. We characterize the retrieval error probability by showing that the vector of similarity margins converges to a multivariate Gaussian distribution, yielding an explicit approximation and computable upper bounds. Numerical results support the analysis, while a separate data-driven evaluation using embedding-based retrieval on real-world data shows that the same importance-aware redundancy principles extend to modern retrieval pipelines. Overall, the results show that assigning higher redundancy to semantically important query features improves retrieval reliability.

==> macros.tex <==
% add macros here

%%%%%%%%%%%%%%%
% Notation (fonts, etc.)
%\newcommand{\Reals}{\mathbb{R}}
%\newcommand{\Naturals}{\mathbb{N}}   % natural numbers 1,2,3,...
\newcommand{\set}[1]{\mathcal{#1}}
\DeclareMathOperator{\supp}{supp}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Mathematical operators, etc.
\renewcommand{\Pr}[1]{\mathbb{P} \left[ #1 \right]}

\newcommand{\EE}[2][]{% expectation
	\ifthenelse{\equal{#1}{}}%
	{\mathbb{E} \left[ #2 \right]}% if #1 is empty
	{\mathbb{E}_{#1} \left[ #2 \right]}% if #2 is not empty
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Re-define the numbering of theorems, lemmas, examples, etc. %%%%%%%
%%\theoremstyle{definition}
\newtheorem{example}{Example}
\newtheorem{remark}{Remark}
\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\sloppy
\allowdisplaybreaks


%%%%%%%%%%%%%%%%%%%%%%
% Proofreading
%\newcommand{\JKL}[1]{\textcolor{red}{$\Rightarrow$ \bf #1 $\Leftarrow$}}
%\newcommand{\jj}[1]{\textcolor{black}{#1}}
\newcommand{\SJ}[1]{\textcolor{blue}{#1}}
\newcommand{\todo}[1]{\textbf{TODO: #1}}
\newcommand{\remove}[1]{\textcolor{gray}{#1}}
\newcommand{\note}[1]{\textbf{NOTE: #1}}



==> packages.tex <==
%%%%%
%% Packages:
\usepackage[utf8]{inputenc} 
\usepackage[T1]{fontenc}
\usepackage{url}              % provides \url{...}
%\usepackage{ifthen}          % provides \ifthenelsetha
\usepackage{cite}             % improves presentation of citations

\usepackage[cmex10]{amsmath}  % Use the [cmex10] option to ensure complicance
% with IEEEXplore (see bare_conf.tex)
\interdisplaylinepenalty=1000 % As explained in bare_conf.tex
\usepackage{mleftright}       % fix to wrong spacing of \left-,
\mleftright                   % \middle- \right-commands 

\usepackage{graphicx}         % provides \includegraphics{...} to
% include graphics (pdf format)
\usepackage{booktabs}         % fixes poor spacing in tables and
% provides \toprule, \midrule, \bottomrule
\include{../packages.tex}
\include{../macros.tex}
%\usepackage{algorithmicx}    % provides an algorithmic environment for
% describing algorithms. See
% https://ctan.org/pkg/algorithmicx

%\usepackage[caption=false,font=footnotesize]{subfig}
% provides subnumbering within a
% floating figure or table

%% For arrays and multiple-line equations, use the
%% IEEEeqnarray-environment. See
%%              https://moser-isi.ethz.ch/manuals.html#eqlatex  
%% for instructions.

%% Do NOT use amsthm or hyperref!
%% -IEEEtran provides its own versions of theorems.
%% -IEEEXplore does not accept submissions with hyperlinks

\usepackage[pass]{geometry} % the original layout should be memorized here

% The preceding line is only needed to identify funding in the first footnote. If that is unneeded, please comment it out.
\usepackage{cite}
\usepackage{pgfplots}
\usepackage{csquotes}
\usepackage{amsmath,amssymb,amsfonts,amsthm}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{xcolor, soul}
\sethlcolor{cyan}
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
		T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}
%%%%%%% Other packages %%%%%%%
\usepackage{bm}
\usepackage{enumitem}       % require for description environment
% \usepackage[bottom]{footmisc} % puts the footnote as much to the bottom as possible
%\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{caption}
%\captionsetup{justification=centering}
\usepackage{tikz}
\usepackage[lined,boxed,linesnumbered,ruled,vlined]{algorithm2e}
\usepackage{comment}
\usepackage{balance}
\usepackage[capitalize]{cleveref} % "clever" references with \cref{} (no "Theorem~" needed)
	\crefname{equation}{}{}
	\crefname{theorem}{Theorem}{Theorems}
	\crefname{lemma}{Lemma}{Lemmas}
	\crefname{cor}{Corollary}{Corollaries}
	\crefname{prop}{Proposition}{Propositions}
	\crefname{note}{Note}{Notes}
	\crefname{appsec}{Appendix}{Appendices}
	\crefname{definition}{Definition}{Definitions}
	\crefname{conj}{Conjecture}{Conjectures}
	\crefname{construction}{Construction}{Constructions}
%\usepackage[size=small]{caption}
%\usepackage[size=small,labelformat=simple]{subcaption}
\usepackage{ifthen}% manage which version to show in LaTeX
\newboolean{IncludeRandomWalk} % IncludeRandomWalk stands for "include Appendix C random walk"
%\setboolean{IncludeRandomWalk}{true} 
\setboolean{IncludeRandomWalk}{false}
%\newboolean{SV} % SV stands for "short_version"
%\setboolean{SV}{true} % true for short_version 
%\setboolean{SV}{false} % false for full version
\newboolean{DecreasingLearningRate} % DecreasingLearningRate stands for "decreasing learning rate"
%\setboolean{DecreasingLearningRate}{true} % true for including subsection on decreasing learning rate 
\setboolean{DecreasingLearningRate}{false} % false for NOT including subsection on decreasing learning rate 
\usepackage{nicefrac}  % compact symbols for 1/2, etc.
\usepackage{mathrsfs}  % provides mathscr: Ralph Smith's Formal Script
\usepackage{float}
\usepackage[caption=false,font=footnotesize,labelformat=simple]{subfig}

\usetikzlibrary{shapes, patterns,decorations.text, decorations.pathreplacing}
\renewcommand\thesubfigure{(\alph{subfigure})}


%% add packages here
%\usepackage{pgfpages}
%\usepackage{graphicx}
%\usepackage{graphics}
%\usepackage{setspace}
%\usepackage{color}
%\usepackage{colortbl}
%\usepackage{xcolor}
%\usepackage{multirow}
%\usepackage{array}
%\usepackage{xspace}
%\usepackage{tikz}
%\usetikzlibrary{positioning}
%\usepackage{nicefrac}
%\usepackage{pgfplots}
%\pgfplotsset{compat=1.16}
%\usepackage[absolute,overlay]{textpos}
%\usepackage{ctable}
%\usepackage{mathtools}
%\usepackage{pbox}
%\usepackage[export]{adjustbox}
%\usepackage{amsmath} % improved math formulas
%\usepackage{amssymb} % math symbols
%\usepackage{amsthm} % theorem environments
%\usepackage{thmtools} % extends amsthm with autoref compat. etc.
%\usepackage{bm} % bold math
%\usepackage{csquotes} % context-sensitive quotation
%\usepackage{balance} % balance columns on the final page
%\usepackage{addlines} % add/remove lines from length of a page
%\usepackage[square,sort]{natbib} % use separate citation and bibliography styles
%\usepackage[normalem]{ulem}
%\usepackage{comment}
%\usepackage{standalone} % subfile support
%\usepackage{graphicx}               % Necessary to use \scalebox
%\usepackage{amsmath,amssymb}
